Control- & Task-Aware Optimal Design of Actuation System for Legged Robots using Binary Integer Linear Programming

Athletic robots demand a whole-body actuation system design that utilizes motors up to the boundaries of their performance. However, creating such robots poses challenges of integrating design principles and reasoning of practical design choices. This paper presents a design framework that guides designers to find optimal design choices to create an actuation system that can rapidly generate torques and velocities required to achieve a given set of tasks, by minimizing inertia and leveraging cooperation between actuators. The framework serves as an interactive tool for designers who are in charge of providing design rules and candidate components such as motors, reduction mechanism, and coupling mechanisms between actuators and joints. A binary integer linear optimization explores design combinations to find optimal components that can achieve a set of tasks. The framework is demonstrated with 200 optimal design studies of a biped with 5-degree-of-freedom (DoF) legs, focusing on the effect of achieving multiple tasks (walking, lifting), constraining the mass budget of all motors in the system and the use of coupling mechanisms. The result provides a comprehensive view of how design choices and rules affect reflected inertia, copper loss of motors, and force capability of optimal actuation systems.

==> bin/alternative.tex <==


% One way to think about force control bandwidth is, “which agent is attributable to force generation and impact absorption. Taking humanoid for an example, there are largely two functionally different agents — 1) torso as a huge (passive) lump of mass and  2) legs which is a collection of links and actuators. For instance, if the ground contact impulse pass through torso, it means legs have less chance of absorbing impulse and torso will suffer from sharp oscillations. For limbs to take in all incoming impulse instead of torso, then the actuators should appear as *easier* pathway for the impulse to pass through than torso. To achieve latter, actuators’ reflected inertia should be minimized. This intuitive analysis and following math both confirm my idea of ‘mechanical impact circuitry’.  

% Second way to think about force control bandwidth is to mathematically analyze the bandwidth which was already done in Patrick Wensing’s impact mitigation paper. In high-level, the control bandwidth takes the form of $w_n^2 =k/m_e$ regardless of actuation type whether it be rigid or series elastic. Then the goal would be to *minimize the effective mass $m_e$.* Let me explain that it is.

% Here is representative model of legged robot. Left is rigid actuation and right is SEA (see a small torsional spring is attached to the rotor).


% I say we need to take another leap in machine thinking. Conventional design approaches tend to NOT specify how much torque and velocity is needed at specific timing. However, for machines to be more dynamic and to reason about athletic intelligence, we better do so. Assuming that we have simulations of anticipated tasks, rough dynamics and rough morphology of a machine, then we can take these information into design optimization and build compact yet powerful machines.

% The torque and velocity are implicitly coupled their timing. This coupling is useful when you consider the power of motor or actuator, which is the product of torque and velocity. For instance, electric motors usually have limit to dissipate power which is not apparent when you consider power and velocity separately. 





% However, these guidelines do not provide quantitative means to compare design scenarios. This becomes a problem especially when the robot is expected to operate at boundaries of system capability (e.g., low actuator mass budget, high torque requirement, limited power consumption on motors). In this case, a designer's expert knowledge is challenged at multiple facades. First, as to creating robots capable of multiple tasks -- actuation topology (coupling) [TelloCA] -- employing differential coupling be good for jumping, but it is still questionable if it is the right way to build a humanoid for wider sets of tasks. Secondly, as the system size grows (in the number of actuators and joints), making multi-objective decision becomes exponentially difficult job. objectives are nonlinear, with more actuation, the robot can do wider sets of tasks, more candidate designs and simulation becomes more difficult. All combined, investigating all combinations becomes intractable.  
% (For example, a designer needs to make decision between total mass budget of actuators, reflected inertia of the whole system, and power consumption of the entire transmission system.) Third, traditional way of respecting tasks trajectories (torque, velocity) which is to decouple them may not work anymore. Legged robots are expected to run faster and carry more load, and the product of torque and velocity = power could pose a serious treat of thermally damaging a motor.  

% \textbf{Paragraph 12:} Given an example of trade-off between motor mass, reflected inertia, gear ratio, and power consumption. 

% \textbf{Paragraph 2:} This paper presents one way to solve above issues at one-shot. In high-level, 1) decouple task simulation/motion generation and design synthesis 2) reduce the design space with designers expert knowledge and limiting component choices to subsets of readily-available ones in market 3) explicitly calculating quantities or limitations of hardware components. In high-level the design optimization writes as follows



% My idea of transmission optimization is to 1) get trajectories of anticipated tasks (sets of tasks) and 2) come up with a system of motors, reduction and couplings between actuators that is powerful enough to cover the tasks. I believe this hierarchy is more principled than conventional approach, and we could see variation in morphology depending on how we specify the tasks. Moreover, this approach will later enable faster data-driven design. 

